GDPR Anti-Patterns: How Design and Operation of Modern Cloud-scale Systems Conflict with GDPR

In recent years, our society is being plagued by unprecedented levels of privacy and security breaches. To rein in this trend, the European Union, in 2018, introduced a comprehensive legislation called the General Data Protection Regulation (GDPR). In this article, we review GDPR from a systems perspective, and identify how the design and operation of modern cloud-scale systems conflict with this regulation. We illustrate these conflicts via six GDPR anti-patterns: storing data without a clear timeline for deletion; reusing data indiscriminately; creating walled gardens and black markets; risk-agnostic data processing; hiding data breaches; making unexplainable decisions. Our findings reveal deep-rooted tussle between GDPR requirements and how cloud-scale systems that process personal data have evolved in the modern era. While it is imperative to avoid these anti-patterns, we believe that achieving compliance requires comprehensive, grounds up solutions; anything short would amount to fixing a leaky faucet in a sinking ship.

==> discussion.tex <==
\section{Discussion}
\label{sec-discussion}

%What is our hypothesis, and what feedback are we looking for
%Controversial points of the paper
%open issues not addressed 
%Limitations: We do not prescribe policies or mechanisms for compliance.

